Towards Modeling and Influencing the Dynamics of Human Learning

Humans have internal models of robots (like their physical capabilities), the world (like what will happen next), and their tasks (like a preferred goal). However, human internal models are not always perfect: for example, it is easy to underestimate a robot's inertia. Nevertheless, these models change and improve over time as humans gather more experience. Interestingly, robot actions influence what this experience is, and therefore influence how people's internal models change. In this work we take a step towards enabling robots to understand the influence they have, leverage it to better assist people, and help human models more quickly align with reality. Our key idea is to model the human's learning as a nonlinear dynamical system which evolves the human's internal model given new observations. We formulate a novel optimization problem to infer the human's learning dynamics from demonstrations that naturally exhibit human learning. We then formalize how robots can influence human learning by embedding the human's learning dynamics model into the robot planning problem. Although our formulations provide concrete problem statements, they are intractable to solve in full generality. We contribute an approximation that sacrifices the complexity of the human internal models we can represent, but enables robots to learn the nonlinear dynamics of these internal models. We evaluate our inference and planning methods in a suite of simulated environments and an in-person user study, where a 7DOF robotic arm teaches participants to be better teleoperators. While influencing human learning remains an open problem, our results demonstrate that this influence is possible and can be helpful in real human-robot interaction.

==> sections/intro_notes.tex <==
\section{Introduction}
% \item Human-robot interaction is rapidly growing, from autonomous vehicles that are deployed in cities and driving around people \cite{}, to robots assisting humans with daily living \cite{}. 
% \item Synthesizing robot behavior has been a key challenge, and to-date a lot of research has focused on how humans---and the data they generate---can teach robots to be better independent agents, teammates, and collaborators (IRL, LfD, prediction etc.). 
% \item Implicit in these works is that humans know best and robots should always learn from human input. 
% \item However, this is not always true. 

% ==== INTRO ==== %
As robots become more capable, humans will increasingly interact with robots in their daily lives. 
For example, consider teleoperating an assistive robot arm to perform daily living tasks like throwing away trash, picking up objects from the table, or stirring a pot of soup. 
To date, a lot of work has focused on how robots can infer an end-user's goal (e.g., which bin they want to throw trash into) \cite{jain2019probabilistic}, their task preferences (e.g., how the human wants to pick up objects) \cite{pfeiffer2016predicting}, or their understanding of physics (e.g., the human's internal model of the robot's dynamics) \cite{reddy2018you}. 

In these paradigms, we typically assume that a human's internal model of the world, their preferences, and their goals are \textit{accurate} and \textit{static}. 
However, robots become more capable, the robot will sometimes know best! 

% option 1:
% However, as humans repeatedly interact with robots, they implicitly or explicitly \textit{learn} about the robot, physical aspects of the world, or their preferences about tasks or goals. 

% as robots become more capable, the robot will sometimes know best! 
% for example, blablabla. 
% this raises an interesting question for robot autonomy -- can the robot teach / influence the human to align the human's internal model? 
% in order to influence a human's understanding, the robot needs to understand how humans learn / update their internal models of the world. 
% in this work, our key idea is to model human learning as a nonlinear dynamical system, where the human's parameter estimate is part of the state, and the observations they receive control the parameter evolution
% using demonstrations of human behavior which naturally exhibit learning (e.g., initial trails of the human teleoperating a robot they have never interacted with before), we can infer the human's learning dynamics.
% we formulate a maximum likelihood estimation problem and approximate the intractable inference problem to obtain a differentiable learning objective that is not only efficient to solve via gradient-based optimization, but is also compatible with deep neural network representations of the human learning dynamics.
% 



% ======================================%
% As humans repeatedly interact with robots, humans implicitly or explicitly \textit{learn} about the robot, physical aspects of the world, or their preferences about the tasks. 
% For example, imagine that you are teleoperating a robot manipulator for the first time (Figure \ref{}). Initially, you have a misconceived notion of its physics \cite{}
% % In fact, there is evidence that humans have misconceived notions of physics \cite{}, may be uncertain about ways to do tasks \cite{}, or may not understand why other agents behave the way they do \cite{}. 
% Open challenges in robot teleoperation \cite{rea2022still} include leveraging how humans learn to teleoperate. 
% In this work we are interested in the question: can robots---and the data they generate---teach humans how to be better collaborators? 
% The major challenge is modelling how people learn. 
% Our key idea is to
% \begin{quote}
%     \textit{model human learning as a nonlinear dynamical system, where the human's parameter estimate is part of the state, and the observations they receive control the parameter evolution.} 
% \end{quote}
% Using demonstrations which exhibit human learning, we formulate a maximum likelihood estimation problem to infer the human's learning dynamics. 
% We approximate the intractable inference problem to obtain a differentiable learning objective that is not only efficient to solve via gradient-based optimization, but is also compatible with deep neural network representations of the human learning dynamics. 
% We then pose and solve a novel constrained planning problem which demonstrates that, if the robot knows how humans learn, the robot can automatically \textit{influence} the human's learning. 
% \textcolor{red}{robots can align their internal models with humans if they plan with the human's learning dynamics.}
% We highlight the benefits of our human learning dynamics model in robot planning to teach the human a better mental model of the robot's physics and influence the human's task preferences. 
%     % \item Additionally, we show that if the robot has access to how the humans learn, it can control the observations the human sees to influence them. 
%     % \item We propose an optimization-based approach to estimate human learning dynamics from demonstrations which exhibit human learning.
%     % \item Then, we integrate these human learning dynamics into robot motion planning as a way for the robot to automatically synthesize behaviors which teach humans to be better collaborators. 
% We first evaluate our framework with simulated humans in order to validate the effecetiveness of our human learning dynamics model as well as the effect of robot teaching.
% We conducted a user study with a Kinova Jaco 7DOF arm where the robot teaches the human to be a more effective teleoperator. 


==> sections/pomdp_formalism.tex <==
\section{Formalism}
% Formalizing robot influence over human learning

In this section we formalize the problem of robot influence over human learning. 

\medskip
\noindent \textbf{Notation.}
Let $\jointstate \in \mathbb{R}^{n}$ be the robot's physical state. The human interacts with the robot by taking actions $\uH \in \mathbb{R}^{m_\mathrm{H}}$, for example, through a joystick or a gesture-based interface.
The robot can also take actions, $\uR \in \mathbb{R}^{m_\mathrm{R}}$, like commanding joint torques or end-effector velocities.
Both the human and robot actions can affect the robot's state, which evolves via the deterministic physical dynamics 
\begin{equation}
\jointstate^{t+1} = \jointdyn(\jointstate^t, \uH^t, \uR^t).
\label{eq:physical_dyns}
\end{equation}

\noindent \textbf{Human internal model.} 
We model the human as having an internal model pararameter, $\param$, which captures a latent aspect of the task that the human is uncertain about but \textit{continuously learns about}. 
Let's go back to our motivating example where the human is teleoperating the robotic manipulator through a gesture-based interface. 
Here, $\param$ can model the human's current estimate of the robot's physical dynamics.
At first, the human may mistakenly believe that the robot doesn't experience any inertia. 
% When planning their action, the human assumes that the robot will behave according to this zero-inertia model. 
However, as soon as the human gestures to move the robot forward, they see the robot lagging behind where they thought the robot would be! 
This observation prompts the human to update their internal model of the robot's physics. 

% In other words, given an observation, the human's \textit{learning dynamics} evolve the human's latent parameter estimate. 
% Or, $\param$ could model the human's current preferences for how they perform a task.

With this in mind, the robot can take actions $\uR$ to \textit{influence} the human's internal model. For example, the robot could use its actions to change the next state, and cause the human to quickly understand that the robot has more inertia than the human originally thought.
The challenge is that the robot needs to understand \textit{how} the human updates their internal model in response to new observations. 

% The human optimizes a reward function, $R_\mathrm{H}(\jointstate, \uH; \param)$, which depends on the current state, the human's action, and their internal parameter $\param$. 

\medskip 
\noindent \textbf{Formalism.} We model the problem of robot influence over human learning as an instance of a partially observable Markov decision process (POMDP).
The human's internal model, $\param$, is a hidden part of the state that the robot receives observations about through the human's actions. 
Formally, a POMDP is a tuple of $<S, U_\mathrm{R}, Z, T, O, r_\mathrm{R}>, \gamma$:
\begin{itemize}
    \item $S : X \times \Theta_\mathrm{H}$ is the set of state which includes both the physical robot state $\jointstate$ as well as the human internal model parameter: $s = (\jointstate, \param)$.
    \item $U_\mathrm{R}$ is the set of robot actions. 
    \item $Z$ is the observations (i.e., the human's actions $\uH \in U_\mathrm{H}$).
    \item $T(s^t, \uH^t, \uR^t, s^{t+1})$ is the transition function. It evolves the physical state $\jointstate$ as well as the human's internal model parameter $\param$. 
    \item $O(z^t \mid s^t)$ is the robot's observation distribution.
    \item $r_\mathrm{R}(s, \uR)$ is the robot's reward function.
    \item $\gamma \in (0,1]$ is the discount factor. 
\end{itemize}


\medskip 
\noindent \textbf{Observation model.}
% \textbf{Human action model.}
Recall that the robot's observations are the human's actions $\uH$. Thus, the observation model captures the probability of seeing a human take an action, given the physical state of the robot $\jointstate$ and the human's internal model $\param$. 
To construct this observation distribution, we model the human optimizing a reward function, $R_\mathrm{H}(\jointstate, \uH; \param)$, which depends on the current state, the human's action, and their internal parameter $\param$. 

Following prior works \cite{ziebart2008maximum, waugh2010inverse, levine2012continuous, baker2009action}, we model the human as a noisily-optimal actor:
\begin{align} 
    & \mathbb{P}(\uH \mid  \jointstate; \param) = \frac{e^{Q_\mathrm{H}(\jointstate, \uH;\param)}}{\int_{\Tilde{u}} e^{Q_\mathrm{H}(\jointstate, \Tilde{u};\param)}d\Tilde{u}}, 
    \label{eq:human_policy}
\end{align}
where the optimal state-action value at the current timestep is denoted by $Q_\mathrm{H}(\jointstate, \uH; \param)$ and $\jointstate$ is the current state, $\uH$ is the human action, and $\param$ the human's current parameter estimate. 

% We make two key assumptions about how the human plans with this reward function. 
We make two key assumptions in this model. First, the human does not explicitly account for the actions $\uR$ the robot could take. 
Instead, the human reacts to the current state $\jointstate$, which \textit{implicitly} captures the effect of any additional robot actions that change the state. 
This models scenarios where the human is doing the task on their own, or where the human is not aware of how the robot is providing guidance. 
Second, when the human is planning their action, we assume that they separate the estimation of $\param$ from policy generation; in other words, the human keeps their parameter $\param$ constant along their planning horizon.

\medskip 
\noindent \textbf{Transition function.} A key modelling challenge lies in the transition function that maps from $s^t = (\jointstate^t, \param^t)$ to $s^{t+1} = (\jointstate^{t+1}, \param^{t+1})$. 
When the robot plans, it needs to reason over both the physical dynamics $\jointstate^t$, but also the human's learning dynamics that evolve $\param^t$ to $\param^{t+1}$. Mathematically, the robot needs access to two functions:
\begin{equation}
    T(s^t, \uH^t, \uR^t, s^{t+1}) = 
    \begin{bmatrix}
    \jointdyn(\jointstate^t, \uH^t, \uR^t) \\ 
    \paramdyn(\param^t, \jointstate^{t}, \uH^{t}, o_\mathrm{H})
    \end{bmatrix},
\end{equation}
where $f$ are the physical dynamics from Equation~\eqref{eq:physical_dyns} and $\paramdyn$ are the \textit{human's learning dynamics} that evolve their internal parameter $\param$. 
We assume that both the physical state and the human's internal model evolve deterministically. 
Here, $o_\mathrm{H} = g(\jointstate^{t}, \uH^{t},\uR^t)$ is the human's observation function. \abnote{I think it would be better if we somehow clarified the notation about $o_\mathrm{H}$..}
% that human uses to up


Here we are faced with the question \textit{``What $\paramdyn$ models the human's learning dynamics?''}
Prior work has always assumed that people have fixed internal models \cite{sadigh2016planning, kitani2012activity} (i.e., $\paramdyn$ is the identity function), or that people learn in a specific way such as via a Bayesian update \cite{reddy2020assisted} (i.e., $\paramdyn$ computes a posterior over $\param$).

Instead of assuming a particular model of how people learn, we seek to \textit{infer} a model of $\paramdyn$, and then enable a robot to plan over this model to influence how humans learn.
% The physical state evolves via $\jointstate^{t+1} = \jointdyn(\jointstate^t, \uH^t, \uR^t)$. The human's latent parameter evolves via $\param^{t+1} = \paramdyn(\param^0, \jointstate^{0:t}, \uH^{0:t}, o_\mathrm{H}^{0:t+1})$.
